Graph-Based Reductions for Parametric and Weighted MDPs

We study the complexity of reductions for weighted reachability in parametric Markov decision processes. That is, we say a state p is never worse than q if for all valuations of the polynomial indeterminates it is the case that the maximal expected weight that can be reached from p is greater than the same value from q. In terms of computational complexity, we establish that determining whether p is never worse than q is coETR-complete. On the positive side, we give a polynomial-time algorithm to compute the equivalence classes of the order we study for Markov chains. Additionally, we describe and implement two inference rules to under-approximate the never-worse relation and empirically show that it can be used as an efficient preprocessing step for the analysis of large Markov decision processes.

==> intro.tex <==
\begin{abstract}
In order to make model checking of large Markov decision processes (MDPs) --- and extensions thereof --- more efficient, it is necessary to reduce them in size. 
For this purpose, we extend the never-worse relation (NWR) from Le Roux and P\'{e}rez to weighted and parametric MDPs. 
The weighted case allows us to reduce the size of MDPs with a mean-payoff objective function. We show that this the natural decision problem, i.e. whether two states are in relation, reduces to the same problem for the non-weighted MDPs and is thus coNP-complete. 
For parametric MDPs, deciding the NWR turns out to be coETR-complete.
In view of the relatively high complexity of computing the exact relations, we also studied efficient algorithms for under-approximating the NWR. We have  implemented the latter in a prototype tool and applied it to a number of common benchmarks. Our experiments show that these under-approximations can already reduce the size of MDPs by \textcolor{red}{insert order of magnitudes}.

\keywords{Markov decision process \and Probabilistic model checking \and State-space reduction.}
\end{abstract}

\section{Introduction}
\textcolor{red}{revisit intro}

The Never-Worse Relation (NWR) compares the maximum reachability probability (to a fixed target) of some state to that of a set of states. That is, we say $W\subseteq V$ is never worse than $v\in V$ (denoted by $v\trianglelefteq W$) if, for each possible probability distribution that could be assigned to the actions of the MDP
there is at least one vertex in $W$ whose value is at least as large as the value of $v$. Parametric MDPs are MDPs in which the probabilities of edges from actions to states are replaced by polynomials and the probabilities are obtained by assigning values to the variables in the polynomials throughout the MDP.

It was shown in \cite{NWR_paper} that deciding the NWR was \textCoNP-complete for regular MDPs (i.e. ones in which the edges from actions can take any value in the range $(0,1]$ and must add up to $1$). Junges et al in \cite{junges2021} showed various results for simple parametric MDPs (the parameters can only be of the form $x$ or $1-x$), most of which can be used to show similar upper and lower bounds for the never worse relation in this model.

Weighted MDPs are stochastic models which have multiple target states, each of which have a different reward for hitting them. In this paper, we first show that for any weighted MDP, we can construct a non weighted MDP that preserves all the never-worse relations of the original weighted MDP. We then show co-ETR completeness of deciding the never-worse relation for parametric MDPs. Finally, since deciding the never-worse relation is co-NP complete and co-ETR complete in the non-parametric and parametric case respectively, we propose an efficient way to under-approximate the NWR and hence, reduce the size of the MDP. \textcolor{red}{(TODO: add implementation results once they are done)}

